Should We Even Optimize for Execution Energy? Rethinking Mapping for MAGIC Design Style

Memristor-based logic-in-memory (LiM) has become popular as a means to overcome the von Neumann bottleneck in traditional data-intensive computing. Recently, the memristor-aided logic (MAGIC) design style has gained immense traction for LiM due to its simplicity. However, understanding the energy distribution during the design of logic operations within the memristive memory is crucial in assessing such an implementation's significance. The current energy estimation methods rely on coarse-grained techniques, which underestimate the energy consumption of MAGIC-styled operations performed on a memristor crossbar. To address this issue, we analyze the energy breakdown in MAGIC operations and propose a solution that utilizes mapping from the SIMPLER MAGIC tool to achieve accurate energy estimation through SPICE simulations. In contrast to existing research that primarily focuses on optimizing execution energy, our findings reveal that the memristor's initialization energy in the MAGIC design style is, on average, 68x higher. We demonstrate that this initialization energy significantly dominates the overall energy consumption. By highlighting this aspect, we aim to redirect the attention of designers towards developing algorithms and strategies that prioritize optimizations in initializations rather than execution for more effective energy savings.

==> Sections/rw.tex <==
Memristive devices (memristors) are two-terminal passive devices with variable resistance, initially proposed by Chua in 1971~\cite{chua}. Memristors have non-volatile resistance states, which is a function of applied voltage amplitude and its duration, alternatively integral over time of the applied voltage across them. The maximum and minimum resistance values of memristors are represented by a low resistive state (LRS) and a high resistive condition (HRS), which are mapped to logic states '0' and '1', respectively. Considering these states, Boolean logic operations can be performed by arranging the memristive devices into crossbar connections and applying different voltages across them. Numerous models have been proposed in the literature to characterize the memristive devices for SPICE simulation. VTEAM model~\cite(vteam) is one of the models that can characterize a variety of different memristive technology and hence being used for this work. 

\emph{MAGIC:} MAGIC is a stateful logic technique to implement logic operations using memristive devices, where inputs and outputs of logic operations are stored in the resistive states of memristors. Figure 1(a) shows the NOR and NOT gate implementation using memristors. An output memristor, $M_{out}$, is initialized to LRS, and it changes the state from LRS to HRS based on the input state stored in $M{in1}$ and $M{in2}$. NOR and NOT operation utilizes three (two input, one output) and two memristors (one input, one output) in a single operation. However, when devices are connected in a crossbar structure, the unselected cell must be isolated from the operation. Figure (b) shows MAGIC implementation in a crossbar, where red memristors are unselected and isolated by applying an isolation voltage.

Figure 2(b) shows the implementation of MAGIC NOR operation in a 1x6 crossbar. In a single time sequence or operation cycle, only three memristors are active (two for inputs, marked in black, and one for output, marked in green). The other three inactive memristors (marked in red) need to be isolated from the network for the functional correctness of the operation. The isolation voltage also solves the purpose of undesired switching of inactive devices. However, applying isolation voltages consumes energy per operation, which needs to be considered for accurate energy estimation of an application. 

\emph{SIMPLER Mapping:}
We take the Verilog design implementation as the SIMPLER tool's input. MAGIC design style-based NOR and NOT implementations can be mapped to a memristor crossbar. 
Considering the MAGIC NOT and NOR implementation, the SIMPLER tool synthesis the Verilog design to NOT and NOR netlist. This output is further used to map the NOR and NOT logic gates to the crossbar, and the output of the same is stored in a .json file. 

-- Present techniques to calculate the energy \\
